Wide Compression: Tensor Ring Nets

Deep neural networks have demonstrated state-of-the-art performance in a variety of real-world applications. In order to obtain performance gains, these networks have grown larger and deeper, containing millions or even billions of parameters and over a thousand layers. The trade-off is that these large architectures require an enormous amount of memory, storage, and computation, thus limiting their usability. Inspired by the recent tensor ring factorization, we introduce Tensor Ring Networks (TR-Nets), which significantly compress both the fully connected layers and the convolutional layers of deep neural networks. Our results show that our TR-Nets approach {is able to compress LeNet-5 by $11\times$ without losing accuracy}, and can compress the state-of-the-art Wide ResNet by $243\times$ with only 2.3\% degradation in {Cifar10 image classification}. Overall, this compression scheme shows promise in scientific computing and deep learning, especially for emerging resource-constrained devices such as smartphones, wearables, and IoT devices.

==> 4TRN.tex <==
\section{Tensor Ring Nets (TRN)}
%\input{FCL_C}
In this paper,  $\mathscr{X} \in \mathbb{R}^{I_1 \times \cdots \times I_d}$ is a $d$ mode tensor with $\prod_{i=1}^d I_i$ degrees of freedom.
%with $I_{i: i=1,\cdots, d}$ along each mode $i$ is represented by calligraphic letters $\mathscr{X} \in \mathbb{R}^{I_1 \times \cdots \times I_d}$.
A \emph{tensor ring decomposition} factors  $\mathscr X$  into $d$ independent $3$-mode tensors, $\mathscr{U}^{(1)},\ldots,\mathscr{U}^{(d)}$
such that each entry inside the tensor $\mathscr{X}$ is represented as
\begin{equation}
\mathscr{X}_{i_1, \cdots, i_d} = \sum_{r_1,\cdots,r_d}\mathscr{U}^{(1)}_{r_d, i_1, r_1}\mathscr{U}^{(2)}_{r_1, i_2, r_2} \cdots \mathscr{U}^{(d)}_{r_{d-1}, i_d, r_d}
\label{eq:tensor_net_decomp}
\end{equation}
where $\mathscr U^{(i)} \in \mathbb{R}^{r \times I_i \times r}$ (and each $j$ is summed from 1 to $r$).
Under this low-rank factorization, the number of free parameters is reduced to $r^2\sum_{i=1}^{d} I_i$ in the tensor ring factor form,  which is significantly less than $\prod_{i=1}^d I_i$ in $\mathcal{X}$.
%\red{and for low enough $r$ and high enough $d$, is a significant reduction in complexity.}


\blue{
	For notational ease, define $\decomp(\mathscr U)$ as the operation \eqref{eq:tensor_net_decomp} where
	 $\mathscr U = (\mathscr{U}^{(1)}, \ldots, \mathscr{U}^{(d)})$.
	 (We assume that $\mathscr X$ always has such a low-rank decomposition whenever $\decomp(\mathscr X)$ is called.)
	 Additionally,
for $1 \leq k < j \leq d$, define \merge~ as
\begin{multline*}
	\merge( \mathbf{\mathscr U} ,k, j) :=\\ \sum_{r_k,\cdots,r_j}\mathscr{U}^{(k)}_{r_{k-1}, i_k, r_k}\mathscr{U}^{(k+1)}_{r_k, i_{k+1}, r_{k+1}} \cdots \mathscr{U}^{(j)}_{r_{j-1}, i_j, r_j},
\end{multline*}
resulting in an order $r \times I_k\times I_{k+1} \times \cdots \times I_j \times r$ tensor,
and \construct~ as
\[
\construct(\mathbf{\mathscr U} ) = \sum_{r_d}\merge(\mathbf{\mathscr U} , 1,d)_{r_d,\cdots,r_d}
\]
resulting in  an order $I_1\times I_2 \times \cdots \times I_d$ tensor.
}



%Since majority of parameters in the deep neural networks, either from fully connected layers or convolutional layers, are in the tensor form, thus  TRN enable capability of compressing deep neural networks.




%Figure \ref{fig:decomp_diagrams} gives the \red{xx} representation of this multiplication operation, \red{such as previously used in xxx}. Here, nodes correspond to tensors, edges between nodes show multiplication along a dimenension, and the remaining dangling edges give the order and dimension of the final product. 

%\begin{figure}
%	\includegraphics[width=5in]{tensor_decomp_diagrams.png}
%	\label{fig:decomp_diagrams}
%\end{figure}


The number of flops for a \construct~  depends on the sequence of merging $\mathcal{U}^{(i)}, i=1,\cdots,d$. 
\red{When $d$ is small, typically $3$ as the scenario we consider in the paper, we {\bf sequentially} merging $\mathcal{U}^{(i)}$ and obtain the number of flops to be $2r^3I_1I_2 +2r^2I_1I_2I_3$. 
When $d$ is large, a {\bf hieratically} merging approach is applied. For instance when $d=4$, the number of flops for hieratically merging is $2r^3I_1I_2+2r^3I_3I_4 +2 I_1I_2I_3I_4r^2$.}
%The number of flops required for a \construct~is $r^d (d-1)$.

\blue{[YS: I fixed some mistakes, but I'm still not geting the same flop count as you.
	If we don't consider any intermediary factorizations, will this blue calculation be correct? 
	After we resulve this, we can move the blue part to appendix for clarity as an extended example.]
	
\paragraph{Merge ordering}
Consider, for example, trying to compute $\merge(\U,1,4)$. This operation can be computed as either sequentially with $r^3I_3I_4 + r^3I_2I_3I_4+r^{\color{red} 2}I_1I_2I_3I_4$ flops
\[
\sum_{r_1}\mathscr{U}^{(1)}_{r_0, i_1, r_1}\left(\sum_{r_2}\mathscr{U}^{(2)}_{r_2, i_2, r_2}\left(\sum_{r_3}\mathscr{U}^{(3)}_{r_2, i_3, r_3}\mathscr{U}^{(4)}_{r_3, i_4, r_4}\right)\right)
\]
or hierarchically with $r^3(I_1I_2+I_3I_4) + r^{\color{red} 2}I_1I_2I_3I_4$ flops
\[
\sum_{r_2} \left(\sum_{r_1}\mathscr{U}^{(1)}_{r_0, i_1, r_1}\mathscr{U}^{(2)}_{r_1, i_2, r_2}\right) 
\left(\sum_{r_3}\mathscr{U}^{(3)}_{r_2, i_3, r_3}\mathscr{U}^{(4)}_{r_3, i_4, r_4}\right).
\]
More generally, for a sequential method, the flop count is
\[
\textbf{seq}(\mathscr{U}^{(1)},\ldots, \mathscr{U}^{(d)}) :=r^3 \sum_{i=2}^{d-1} \prod_{k=i}^d I_k + r^{\color{red} 2} \prod_{k=1}^d I_k 
\]
flops, or if $I_1 = \cdots = I_d = \bar I$ 
\[
r^3 (d-2)\bar I ^ {(d-i+1)} + r^{\color{red} 2}  \bar I^d \text{ flops.}
\]
For a hierarchical method, the flop count can be computed via a  minimum-depth binary tree with $1,\ldots, d$ as nodes and depth $D = \floor(\log_2(d))$, where $\textbf{ch}(i)$ is the set of children of node $i$, $\textbf{leaf}(i)$ is the set of all leaves that are descendants of node $i$,  $L(i)$ is the set of nodes with a minimum of $i$ edges to any leaf in the tree, and $\hat L(i) = \{j\in L(i) \mid |\textbf{ch}(j)| = 2\}$. 
Then the cost is
\begin{multline}
\textbf{hier}(\mathscr{U}^{(1)},\ldots, \mathscr{U}^{(d)}) :=\\\left(r^3 \sum_{i=1}^{D-2} \sum_{j \in \hat L(i) } \prod_{k\in \textbf{leaf}(j)}^d I_k \right)+ r^{\color{red} 2}  \prod_{k=1}^d I_k \text{ flops}
\end{multline}
or if $I_1 = \cdots = I_d = \bar I$ and $d$ is a power of 2,
\[
r^3 \sum_{i=2}^{D-1} 2^{D-i} \bar I^{2^{i-1}}+ r^{\color{red} 2}  \bar I^d \text{ flops.}
\]
Clearly,  if $d$ is small and each of the $I_k$'s are large, a sequential merging order is preferable; conversely, if $d$ is large and each of the $I_k$'s are large, a hierarchical merging is preferable.
}


==> 6Reshaping.tex <==
{\bf Higher-order reshaping:}
In our implementation, in order to achieve better compressibility, we reshape the kernel tensor $\mathcal{K} \in \mathbb{R}^{D_1 \times D_2 \times F_1 \times F_2}$ into higher order tensors 
$\tilde{\mathcal{K}} \in \mathbb{R}^{D_1 \times D_2 \times F_{11} \times F_{12} \times F_{21} \times F_{22}}$  where $F_1 =F_{11}F_{12}$ and $F_2 =F_{21}F_{22}$, to improve the compressibility when the amount of feature maps, $F_1$ and $F_2$, are large. 
Thus, similar to \eqref{eq: TR_Kernel}, the kernel function $\tilde{\mathcal{K}}$ represented via tensor ring factorization is
\begin{equation}
\begin{split}
\tilde{\mathcal{K}}_{d_1,d_2,f_{11},f_{12},f_{21},f_{22}}
&=\\
\sum_{r_1=1}^{R_1}
\sum_{r_2=1}^{R_2}
\sum_{r_3=1}^{R_3}
\sum_{r_4=1}^{R_4}
\sum_{r_5=1}^{R_5}
&\mathcal{U}^{(1)}_{r_1, d_1, d_2, r_2}
\mathcal{U}^{(2)}_{r_2, f_{11}, r_3}
\mathcal{U}^{(3)}_{r_3, f_{12}, r_4}\\
&\mathcal{U}^{(4)}_{r_4, f_{21}, r_5}
\mathcal{U}^{(5)}_{r_5, f_{22}, r_1}.
\end{split}
\end{equation}

The input tensor $\mathcal{X}\in \mathbb{R}^{H_1 \times W_1 \times F_1}$ is reshaped into $\tilde{\mathcal{X}} \in \mathbb{R}^{H_1 \times W_1 \times F_{11} \times F_{12}}$ to match the dimension of the $\tilde{\mathcal{K}}$, and thus the convolution operation in \eqref{eq: Conv} becomes
\begin{equation}
\begin{split}
&\tilde{\mathcal{Y}}_{h_2, w_2, f_{21},f_{22}} = 
 \sum_{d_1=1}^{D_1}\sum_{d_2=1}^{D_2}\sum_{f_{11}=1}^{F_{11}}\sum_{f_{12}=1}^{F_{12}}
\sum_{r_1=1}^{R_1}\sum_{r_2=1}^{R_2}\sum_{r_3=1}^{R_3}
\sum_{r_4=1}^{R_4}\sum_{r_5=1}^{R_5}
\\
&\tilde{\mathcal{X}}_{h'_2, w'_2, f_{11},f_{12}}
\mathcal{U}^{(1)}_{r_1, d_1, d_2, r_2}
\mathcal{U}^{(2)}_{r_2, f_{11}, r_3}
\mathcal{U}^{(3)}_{r_3, f_{12}, r_4}
\mathcal{U}^{(4)}_{r_4, f_{21}, r_5}
\mathcal{U}^{(5)}_{r_5, f_{22}, r_1}.
\end{split}
\end{equation}
We again change the summation sequence and  obtain the results in Table \ref{table: conv_reshape}.
Since 2D convolutional is the same to 3D convolutional when the $3$rd spatial dimension is $1$, thus we show that 
{\bf after reshaping the $4_\text{th}$ order kernel tensor $\mathcal{K}$ to the $6_\text{th}$ order kernel tensor $\tilde{\mathcal{K}}$, a reshaped high order tensor ring layer is equivalent to a block of $5$ convolutional layers,  two 3D convolutional layer with patch $1\times 1\times 1$, followed by one 3D convolutional layer with patch $D_1 \times D_2 \times 1$ using the given stride and patch, and another two 3D convolutional layer with patch $1\times 1\times 1$.}

Comparing to the non-reshaped kernel $\mathcal{K}$, the reshaped kernel $\tilde{\mathcal{K}}$ gives better compression at a small increased cost in computational time.
The reduction in computation ($C_\text{reshape}$) and memory ($M_\text{reshape}$) cost for high order reshaped tensor ring layer are
\begin{equation}\label{eq: MC2}
\begin{split}
&M_\text{reshape} = \frac{D_1D_2F_1F_2}{
\substack{
D_1D_2R_1R_2 + F_{11}R_2R_3 + F_{12}R_3R_4, \\
+F_{21}R_4R_5 +F_{22}R_5R_1}}\\
&C_\text{reshape} = \frac{H_2W_2D_1D_2F_1F_2}{\substack{H_1W_1F_{11}R_3R_4F_{12} + H_1W_1R_4R_2F_{11}R_3 + H_2W_2R_4R_1D_1D_2R_2 \\+H_2W_2R_1F_{21}R_5R_4 +H_2W_2F_{21}F_{22}R_1R_5
}
}.
\end{split}
\end{equation}
Assuming that all the $R$ are the same in both tensor ring layer and high order reshaped tensor ring layer, we note that \eqref{eq: MC2} is different from \eqref{eq: MC1} since the memory cost is reduced by $R^2(F_1 + F_2 -F_{11}-F_{12} -F_{21}-F_{22})$, which is significant when $F_1$ and $F_2$ are large, and the computational cost only increases by $H_1W_1F_{11}R^3 + H_2W_2F_{21}R^3$, which is relative small as compared with $H_1W_1F_{11}F_{12}R^2 + H_2W_2F_{21}F_{22}R^2$.

\input{Table_Conv_reshape}

==> 7FCCompress2.tex <==
\section{Fully Connected Layer Compression}
In feed-forward neural networks, an input feature vector ${\bf x}\in \mathbb{R}^{I}$ is mapped to an output feature vector ${\bf y} = {\bf Ax}\in \mathbb{R}^{O}$ via a fully connected layer ${\bf A}\in \mathbb{R}^{I \times O}$. 
Without loss of generality, $\bf{x}$, $\bf{A}$, and $\bf y$ can be reshaped into higher order  tensors $\mathscr{X}$, $\mathscr{A}$, and $\mathscr {Y}$ with 
\begin{equation}\label{eq: FC}
\mathscr{Y}_{o_1,\ldots, o_{\hat d}} = \sum_{i_1,\ldots,i_{d}}
 \mathcal{A}_{i_1,\ldots, i_{d},o_1,\ldots, o_{\hat d}} \mathcal{X}_{i_1,\ldots, i_{d}}
\end{equation}
where $d$ and $\hat d$ are the modes of $\mathscr{X}$ and $\mathscr{Y}$ respectively, and $i_k$ are summed from $1$ to $I_k$, $o_k$ spanned from 1 to $O_k$, and
\[
\prod_{i=1}^d I_i = I, \quad \prod_{i=1}^{\hat d} O_i = O.
\]
To compress a feed-forward network, we decompose as $\mathscr{U} =\{
\mathcal{U}^{(1)}, \ldots, \mathcal{U}^{(d+{\hat d})}
\}
= \decomp( \mathcal{A}; R, d+{\hat d} )$
and replace $\mathscr A$ with its decomposed version in \eqref{eq: FC}.


\vspace{-.1in}
\paragraph{Computational cost}
The computational cost again depends on the order of merging $\mathscr{X}$ and $\mathscr{U}$.

One naive approach to compute $\mathscr{Y}$ is first constructing $\mathscr{X}$ from $\mathscr{U}$, followed by a feed-forward layer computation, which degrades the computation efficiency by a constant \construct operation of ${\color{red} 2R^3d \sum_{l=1}^{\log_2(d+\hat{d})} \frac{I^{2l}}{2^l}}$ flops.

To reduce the computational cost, a \emph{layer separation} approach is proposed by first using hieratical merging to obtain 
\begin{equation}
\begin{split}
\mathscr{F}^{(1)} &= \merge(\mathscr{U}, 1, d) \in \mathbb{R}^{R \times I_1 \times \cdots \times I_d \times R}\\
\mathscr{F}^{(2)} &=\merge(\mathscr{U}, d+1, d+\hat{d}) \in
\mathbb{R}^{R \times I_{d+1} \times \cdots \times I_{d+\hat{d}} \times R},
\end{split}
\end{equation}
which takes ${\color{red} O}$ flops. 
Replace $\mathscr{A}$ in \eqref{eq: FC} with  $\mathscr{F}^{(1)}$ and $\mathscr{F}^{(2)}$, switch the order of summation, and thus obtain
\begin{equation}\label{eq: FC_Sep}
\begin{split}
&\mathscr{Y}_{o_1,\ldots, o_{\hat d}} \\
&= \sum_{i_1,\ldots,i_{d}}
 \sum_{r_{d+\hat{d}}, r_d} \mathscr{F}^{(1)}_{r_{d+\hat{d}}, i_1,\cdots, i_d, r_d}
 \mathscr{F}^{(2)}_{r_d, i_{d+1},\cdots, i_{d+\hat{d}}, r_{d+\hat{d}}}
 \mathcal{X}_{i_1,\ldots, i_{d}}\\
 &= 
\sum_{r_{d+\hat{d}}, r_d}
(
\sum_{i_1,\ldots,i_{d}}\mathscr{F}^{(1)}_{r_{d+\hat{d}}, i_1,\cdots, i_d, r_d}
\mathcal{X}_{i_1,\ldots, i_{d}}
)
\mathscr{F}^{(2)}_{r_d, i_{d+1},\cdots, i_{d+\hat{d}}, r_{d+\hat{d}}}.
\end{split}
\end{equation}


The summation $\sum_{i_1,\ldots,i_{d}}\mathscr{F}^{(1)}_{r_{d+\hat{d}}, i_1,\cdots, i_d, r_d}
\mathcal{X}_{i_1,\ldots, i_{d}}$
is equivalent to a feed-forward layer of shape $I_1\cdots I_d \times R^2$, which takes $2I_1\cdots I_dR^2$ flops. 
Additionally, the summation over $r_{d+\hat{d}}$ and $r_d$ is equivalent to another feed-forward layer of shape $R^2 \times I_{d+1}\cdots I_{d+\hat{d}}$, which takes $2I_{d+1} \cdots I_{d+\hat{d}}R^2$ flops. 
Such analysis demonstrates that the \emph{layer separation} approach to a FCL in a tensor ring net is equivalent to a low-rank matrix factorization to a fully-connected layer, thus reducing the computational complexity.

Define $P_{\TRFC}$ and $C_{\TRFC}$ as the complexity saving in Parameters(P) and Computation(C), respectively, for the tensor net decomposition over the typical fully connected layer forward propagation. Thus we have
\begin{equation}
P_{\TRFC} = 
\frac{\prod_i^d I_i \prod_j^{\hat d} O_j }{R^2\left(\sum_i^d I_i +\sum_j^{\hat d} O_j\right)}.
\end{equation}
and
\[
C_{\TRFC}= 
\frac{\prod_i^d I_i \prod_j^{\hat d} O_j }
{R^2(\prod_i^d I_i + \prod_j^{\hat d} O_j) + {\color{red} OO}},
\]


==> FCL_C.tex <==
\subsection{Fully Connected Layer Compression}
In the traditional feed-forward networks, assume batch size is $n$ and there are $I^{(\ell)}$ features in the $\ell_\text{th}$ layer, denoted as ${\bf X}^{(\ell)} \in \mathbb{R}^{n \times I^{(\ell)}}$, a Fully Connected (FC) layer takes  ${\bf X}^{(\ell)}$ as input and outputs a ${\bf X}^{(\ell+1)} \in \mathbb{R}^{n \times I^{(\ell+1)}}$ via applying rectified linear units (ReLU) \cite{glorot2011deep} after a linear transformation ${\bf W}^{(\ell)} \in \mathbb{R}^{I^{(\ell)} \times I^{(\ell+1)}}$,
\begin{equation}
{\bf X}^{(\ell+1)} = \text{ReLU}({\bf X}^{(\ell)} {\bf W}^{(\ell)} ),
\end{equation}
where the FC layer takes $I^{(\ell)} I^{(\ell+1)}$ parameters.  
\begin{equation}
{\bf X}^{(\ell+2)} = \text{ReLU}(\text{ReLU}({\bf X}^{(\ell)} {\bf W}^{(\ell)} ){\bf W}^{(\ell +1)} ),
\end{equation}

\input{Fig1}
In the proposed Fully Connected Tensor Ring Nets (FC-TRN), ${\bf X}^{(\ell)}$ is first reshaped into a higher order tensor $\mathscr{X}^{(\ell)} \in \mathbb{R}^{n \times I_1^{(\ell)} \times I_2^{(\ell)} \times \cdots \times I_d^{(\ell)}}$, and a linear transformation $\mathscr{W}^{(\ell)} \in \mathbb{R}^{(I_1^{(\ell)} \times I_2^{(\ell)} \times \cdots \times I_d^{(\ell)}) \times (I_1^{(\ell+1)} \times I_2^{(\ell+1)} \times \cdots \times I_d^{(\ell+1)})}$ maps $\mathscr{X}^{(\ell)}$ to $\mathscr{X}^{(\ell+1)} \in \mathbb{R}^{n \times I_1^{(\ell+1)} \times I_2^{(\ell+1)} \times \cdots \times I_d^{(\ell+1)}}$, as described in Fig.\ref{FC} that gives
\begin{equation}
\mathscr{X}^{(\ell+1)} = \text{ReLU}(\mathscr{X}^{(\ell)} \mathscr{W}^{(\ell)}).
\end{equation}
Note that the neural networks have not been compressed since $I^{(\ell)} = \prod_{i=1}^d I_i^{(\ell)}$, and the tensor operation is equivalent to the matrix operation. Thus till now the reshaping operation only converts a matrix format into a tensor format. 

FC-TRN compresses the FC layer via factorizing $\mathscr{W}^{(\ell)}$ into $2d$ tensor ring factors $\mathscr{U}_{i:i=1,\cdots, d}^{(\ell)} \in \mathbb{R}^{r \times I_i^{(\ell)} \times r}$ and $\mathscr{U}_{i=1, \cdots, d}^{(\ell+1)} \in \mathbb{R}^{r \times I_i^{(\ell+1)} \times r}$, thus 
\begin{equation}
\mathscr{W}^{(\ell)} = \mathscr{U}_1^{(\ell)} \cdots \mathscr{U}_d^{(\ell)} \mathscr{U}_d^{(\ell+1)} \cdots \mathscr{U}_1^{(\ell + 1)}. 
\end{equation}

We note that reshaping low order data into higher order tensors is a common practice in the literation \cite{wang2017efficient,novikov2015tensorizing} and has demonstrated the improved expressive power in data representation. In this paper, we will utilize the such operation to represent the FC layer more efficiently and further analyze the intuition to reshape the data into higher order tensors. 
\input{Fig2}

==> Fig1.tex <==
\begin{figure}[t]
\begin{tikzpicture}
    \node[draw, shape=circle] (v0) at (0,0) {$\mathscr{X}^{(\ell)}$};
    \node[draw, shape=circle] (v1) at (-2.5,-2) {$\mathscr{U}_1^{(\ell)}$};
    \node[draw, shape=circle] (v2) at (-1,-2) {$\mathscr{U}_2^{(\ell)}$};
    \node[draw, shape=circle] (v3) at (1,-2) {$\mathscr{U}_3^{(\ell)}$};
    \node[draw, shape=circle] (v4) at (2.5,-2) {$\mathscr{U}_4^{(\ell)}$};
    \node[draw, shape=circle] (v11) at (-2.5,-4) {$\mathscr{U}_1^{(\ell)}$};
    \node[draw, shape=circle] (v12) at (-1,-4) {$\mathscr{U}_2^{(\ell)}$};
    \node[draw, shape=circle] (v13) at (1,-4) {$\mathscr{U}_3^{(\ell)}$};
    \node[draw, shape=circle] (v14) at (2.5,-4) {$\mathscr{U}_4^{(\ell)}$};
    % output edge
    \draw[thick, label=below:{v14}] (-2.5,-4.55) -- node[left] {$I_1^{(\ell+1)}$} (-2.5,-5.5); 
    \draw[thick, label=below:{v13}] (-1,-4.55) --    node[left] {$I_2^{(\ell+1)}$}  (-1,-5.5);
    \draw[thick, label=below:{v12}] (1,-4.55) --     node[left] {$I_3^{(\ell+1)}$}(1,-5.5);
    \draw[thick, label=below:{v11}] (2.5,-4.55) --  node[left] {$I_4^{(\ell+1)}$}(2.5,-5.5);
    \draw[thick, label=above:{v0}] (0,.5) --  node[left] {$n$}(0,1.5);
    % input edge
    \draw [thick] (v0) -- node[left] {$I_1^{(\ell)}$} (v1);
    \draw [thick] (v0) -- node[left] {$I_2^{(\ell)}$}(v2);
    \draw [thick] (v0) -- node[left] {$I_3^{(\ell)}$}(v3); 
    \draw [thick] (v0) -- node[left] {$I_4^{(\ell)}$}(v4);
    % rank edge
    \draw [thick] (v1) --   node[below] {r}(v2);
    \draw [thick] (v2) --   node[below] {r}(v3);
    \draw [thick] (v3) --   node[below] {r}(v4);
    \draw [thick] (v4) --   node[left]      {r}(v14);
    \draw [thick] (v11) -- node[above] {r}(v12);
    \draw [thick] (v12) -- node[above] {r}(v13);
    \draw [thick] (v13) -- node[above] {r}(v14);
    \draw [thick] (v11) --  node[right] {r} (v1) ;   
    {\color{green}
    % mark W
    \draw[dashed, label=below:{v11}] (-3.5, -1.4) -- (3.2, -1.4);
    \draw[dashed, label=below:{v11}] (-3.5, -1.4) -- (-3.5, -4.6);
    \draw[dashed, label=below:{v11}] (-3.5, -4.6) -- (3.2, -4.6);
    \draw[dashed, label=below:{v11}] (3.2, -4.6) --  node[right] {$\mathscr{W}^{(\ell)}$}(3.2, -1.4);
    }
    % mark X_l
    {\color{blue}
    \draw[dashed, label=below:{v11}] (-3.5, 1.6) -- (3.2, 1.6);
    \draw[dashed, label=below:{v11}] (-3.5, -.6) -- (-3.5, 1.6);
    \draw[dashed, label=below:{v11}] (-3.5, -.6) -- (3.2, -.6);
    \draw[dashed, label=below:{v11}] (3.2, -.6) --  node[right] {$\mathscr{X}^{(\ell)}$}(3.2,1.6);
    }
    % mark X_l+1
     {\color{red}
    \draw[dashed, label=below:{v11}] (-3.7, 1.7) -- (4.1, 1.7);
    \draw[dashed, label=below:{v11}] (-3.7, -5.3) -- (-3.7, 1.7);
    \draw[dashed, label=below:{v11}] (-3.7, -5.3) -- (4.1, -5.3);
    \draw[dashed, label=below:{v11}] (4.1, -5.3) --  node[right] {$\mathscr{X}^{(\ell+1)}$}(4.1, 1.7);
    }
    \end{tikzpicture}
 \centering
 \caption{Tensor Network Representation: FC-TRN($d=4$). 
    %$\mathscr{W}^{(\ell)} \in \mathbb{R}^{I_1^{(\ell)} \times I_2^{(\ell)} \times I_3^{(\ell)} \times I_4^{(\ell)} \times I_1^{(\ell + 1)} \times I_2^{(\ell + 1)} \times I_3^{(\ell + 1)} \times I_4^{(\ell + 1)} }$, 
    %$\mathscr{X}^{(\ell)} \in \mathbb{R}^{_1^{(\ell)} \times I_2^{(\ell)} \times I_3^{(\ell)} \times I_4^{(\ell)}}$ ,
    %$\mathscr{X}^{(\ell+1)} \in \mathbb{R}^{_1^{(\ell+1)} \times I_2^{(\ell+1)} \times I_3^{(\ell+1)} \times I_4^{(\ell+1)}}$
    }
 \label{FC}
 \vspace{-.2in}
\end{figure}

==> Fig2.tex <==
\begin{figure*}
        \begin{subfigure}[b]{0.12\textwidth}
                \begin{tikzpicture}
  		\matrix (m) [matrix of math nodes, row sep=.6em,column sep=.86em]{
    		& 5& & 7 \\
    		1 & & 3 & \\
    		& 6 & & 8 \\
    		2 & & 4 & \\};
  		\path %[-stealth]
    		(m-1-2) edge (m-1-4) edge (m-2-1) edge [densely dotted] (m-3-2)
    		(m-1-4) edge (m-3-4) edge (m-2-3)
    		(m-2-1) edge [-,line width=6pt,draw=white] (m-2-3) edge (m-2-3) edge (m-4-1)
    		(m-3-2) edge [densely dotted] (m-3-4) edge [densely dotted] (m-4-1)
    		(m-4-1) edge (m-4-3)
    		(m-3-4) edge (m-4-3)
    		(m-2-3) edge [-,line width=6pt,draw=white] (m-4-3) edge (m-4-3);
		\end{tikzpicture}        
	\end{subfigure} 
	\hspace{0in}
         \begin{subfigure}[b]{0.12\textwidth}
                \begin{tikzpicture}
  		\matrix (m) [matrix of math nodes, row sep=.6em,column sep=.6em]{
    		& 13& & 15 \\
    		9 & & 11 & \\
    		& 14 & & 16 \\
    		10 & & 12 & \\};
  		\path %[-stealth]
    		(m-1-2) edge (m-1-4) edge (m-2-1) edge [densely dotted] (m-3-2)
    		(m-1-4) edge (m-3-4) edge (m-2-3)
    		(m-2-1) edge [-,line width=6pt,draw=white] (m-2-3) edge (m-2-3) edge (m-4-1)
    		(m-3-2) edge [densely dotted] (m-3-4) edge [densely dotted] (m-4-1)
    		(m-4-1) edge (m-4-3)
    		(m-3-4) edge (m-4-3)
    		(m-2-3) edge [-,line width=6pt,draw=white] (m-4-3) edge (m-4-3);
		\end{tikzpicture}        
	\end{subfigure}
	\centering
	\hspace{.3in}
	\begin{subfigure}[b]{0.15\textwidth}
		\[
		\begin{bmatrix}
    			{\color{red} {\bf 1} }& 5 & 9  & 13 \\
    			{\color{red}{\bf 2} }& 6 & 10 & 14 \\
    			3 & 7 & 11 & 15 \\
    		 	4 & 8 & 12 & 16
		\end{bmatrix}
		\]
		\caption{}
	\end{subfigure} 
	\begin{subfigure}[b]{0.15\textwidth}
		\[
		\begin{bmatrix}
    			{\color{blue}{\bf 1}} & 5 & {\color{blue}{\bf 9}}  & 13 \\
    			2 & 6 & 10 & 14 \\
    			3 & 7 & 11 & 15 \\
    		 	4 & 8 & 12 & 16
		\end{bmatrix}
		\]
		\caption{}
	\end{subfigure} 
	%
	\begin{subfigure}[b]{0.15\textwidth}
		\[
		\begin{bmatrix}
    			{\color{green} {\bf 1} }& {\color{green} {\bf 5}} & 9  & 13 \\
    			2& 6 & 10 & 14 \\
    			3 & 7 & 11 & 15 \\
    		 	4 & 8 & 12 & 16
		\end{bmatrix}
		\]
		\caption{}
	\end{subfigure} 
	\begin{subfigure}[b]{0.15\textwidth}
		\[
		\begin{bmatrix}
    			{\color{purple}{\bf 1}} & 5 &  9  & 13 \\
    			2 & 6 & 10 & 14 \\
    			{\color{purple}{\bf 3}} & 7 & 11 & 15 \\
    		 	4 & 8 & 12 & 16
		\end{bmatrix}
		\]
		\caption{}
	\end{subfigure} 
	
\caption{Reshaping $4\times4$ Matrix into Tensor $4$-th order tensor.}
\label{M2T}
\vspace{-.1in}
\end{figure*}

==> Table_Conv.tex <==
\begin{table*}[t!]
\begin{tabular}{ |p{9.5cm}||p{3.5cm}|p{3cm}|  }
 \hline
 \multicolumn{3}{|c|}{Convolutional layer in tensor ring nets} \\
 \hline
\[ \text{Formula} \]            			& \[ \text{Method} \] 		& \[ \text{Computation} \]  		 	 \\
 \hline
 %layer 1
 	%\[\mathcal{T}^{(2)} \in \mathbb{R}^{1 \times 1 \times F_1 \times R_3R_2}=\text{reshape}(\mathcal{U}^{(2)} \in \mathbb{R}^{R_2 \times F_1 \times R_3})\]
	%\[\mathcal{Z}^{(1)}_{h'_2, w'_2, r_3r_2} = \sum_{p'=1}^1\sum_{q'=1}^1\sum_{f_1=1}^{F_1} \mathcal{X}_{h'_2, w'_2, f_1}  \mathcal{T}^{(2)}_{p',q', f_1, r_3r_2}\]		
	%\[\tilde{\mathcal{Z}}^{(1)} \in \mathbb{R}^{H_1\times W_1 \times R_3 \times R_2} = \text{reshape}(\mathcal{Z}^{(1)} \in \mathbb{R}^{H_1\times W_1 \times R_3R_2})\]	
	\[\mathscr{P}^{(r_3)}_{h', w', r_2} = \sum_{d_1,d_2=1}^1 \sum_{i=1}^I
\mathscr{X}_{h',w',i}\mathscr{U}^{(2, r_3)}_{d_1,d_2, r_2,i} \]
& \[\text{Conv-2D} \times R\] 
\[(1\times 1 \times I \times R)\] 
\[S=(1,1)\]
\[P=(0,0)\]
&\[HWR^2I\]
\\
\hline
% layer 2
%\[ \mathcal{T}^{(1)} \in \mathbb{R}^{D_1 \times D_2 \times 1 \times R_2 \times R_1} =\text{reshape}(\mathcal{U}^{(1)}\in \mathbb{R}^{R_1 \times D_1 \times D_2 \times R_2 })\]
%\[\mathcal{Z}^{(2)}_{h_2, w_2, r_3, r_1} =  \sum_{d_1=1}^{D_1}\sum_{d_2=1}^{D_2}\sum_{s'=1}^1\sum_{r_2=1}^{R_2}\tilde{\mathcal{Z}}^{(1)}_{h'_2, w'_2, r_3, r_2} \mathcal{T}^{(1)}_{d_1, d_2,s', r_2, r_1}\]
%\[\tilde{\mathcal{Z}}^{(2)}\in \mathbb{R}^{H_2\times W_2 \times R_3R_1} = \text{reshape}(\mathcal{Z}^{(2)} \in \mathbb{R}^{H_2\times W_2 \times R_3 \times R_1})\]
\[\mathscr{Q}^{(r_3)}_{h,w,r} = \sum_{d_1,d_2=1}^D\sum_{r_2=1}^R \mathscr{P}^{(r_3)}_{h',w',r_2} \mathscr{U}^{(1)}_{r_1,d_1,d_2, r_2}\]
& \[\text{Conv-2D} \times R\]
\[(D \times D \times R \times R)\]
\[S=(s,s)\]
\[P=(p,p)\]
&\[HWR^3D^2\]
\\
 \hline
 % layer 3
 %\[\mathcal{T}^{(3)}\in\mathbb{R}^{1 \times 1 \times R_3R_1 \times F_2} = \text{reshape}(\mathcal{U}^{(3)} \in \mathbb{R}^{R_3 \times F_2 \times R_1})\]
%\[\mathcal{Z}^{(3)}_{h_2, w_2,  f_2} = \sum_{p'=1}^1\sum_{q'=1}^1\sum_{r_{31}=1}^{R_3R_1}\tilde{\mathcal{Z}}^{(2)}_{h_2, w_2, r_{31}}\mathcal{T}^{(3)}_{p',q',r_{31}, f_2}\]
\[\mathscr{Z}_{h,w,o} = \sum_{r_3=1}^R\left(\sum_{d_1,d_2=1}^D \sum_{r_1=1}^R\mathscr{Q}^{(r_3)}_{h,w,r_1} \mathscr{U}^{(3, r_3)}_{d_1, d_2, o, r_1}\right)\]
&\[\text{Conv-2D} \times R \]
\[(1 \times 1 \times R \times O)\]
\[S=(1,1)\]
\[P=(0,0)\]
&
\[HWOR^2\]
 \\
 \hline
\end{tabular}
\centering
 \caption{Tensor ring nets analysis.}
 \label{table: conv_eq}
 \vspace{-.1in}
 \end{table*}

==> Table_Conv_reshape.tex <==
\begin{table*}[t!]
\begin{tabular}{ |p{9.5cm}||p{3.5cm}|p{3cm}|  }
 \hline
 \multicolumn{3}{|c|}{Convolutional layer in high order reshaped tensor ring nets} \\
 \hline
\[ \text{Formula} \]            			& \[ \text{Method} \] 		& \[ \text{Computation} \]  		 	 \\
 \hline
 % layer 1
 \[\mathcal{T}^{(3)} \in \mathbb{R}^{1 \times 1\times 1\times F_{12} \times R_{3}R_4} =
 \text{reshape}(\mathcal{U}^{(3)} \in \mathbb{R}^{R_3 \times F_{12} \times R_4})
 \]
\[\mathcal{Z}^{(1)}_{h'_2, w'_2, f_{11}, r_3r_4} =
\sum_{i=1}^1\sum_{j=1}^1\sum_{k=1}^1 \sum_{f_{12}=1}^{F_{12}}\tilde{\mathcal{X}}_{h'_2, w'_2, f_{11},f_{12}}\mathcal{T}^{(3)}_{i,j,k, f_{12}, r_3r_4}\]
\[
\tilde{\mathcal{Z}}^{(1)} \in \mathbb{R}^{H_1 \times W_1 \times R_4 \times F_{11}R_3} =
\text{reshape} (\mathcal{Z}^{(1)} \in \mathbb{R}^{H_1 \times W_1 \times F_1 \times R_3R_4}) 
\]
& \[\text{Conv-3D}\] 
\[(1\times 1 \times 1 \times  F_{12} \times R_3R_4)\] 
\[S=(1,1,1)\]
\[P=(0,0,0)\]
&\[H_1W_1F_{11}R_3R_4F_{12}\]
\\
\hline
% layer 2
\[
\mathcal{T}^{(2)}\in\mathbb{R}^{1\times1\times1\times F_{11}R_3 \times R_2}
\text{reshape}(\mathcal{U}^{(2)}\in \mathbb{R}^{R_2 \times F_{11} \times R_3})
\]
\[
\mathcal{Z}^{(2)}_{h'_2, w'_2, r_4, r_2} = \sum_{p'=1}^{1} \sum_{p'=1}^{1} \sum_{s'=1}^1 \sum_{f_{11}r_3=1}^{F_{11}R_3}
\mathcal{Z}^{(1)}_{h'_2, w'_2, r_4, f_{11}r_3}\mathcal{T}^{(2)}_{p',q', s', f_{11}r_3, r_2 }
\]
\[
\tilde{\mathcal{Z}}^{(2)} \in \mathbb{R}^{H_1 \times W_1 \times R_2 \times R_4} =
\text{reshape}(\mathcal{Z}^{(2)} \in \mathbb{R}^{H_1 \times W_1 \times R_4 \times R_2})
\]
&
\[\text{Conv-3D}\]
\[1\times 1 \times 1 \times F_{11}R_3 \times R_2 \]
\[S=(1,1,1)\]
\[P=(0,0,0)\]
&
\[H_1W_1R_4R_2F_{11}R_3\]
\\
\hline
%layer 3
\[
\mathcal{T}^{(1)} \in \mathbb{R}^{D_1 \times D_2 \times 1 \times R_2 \times R_1} =
\text{reshape}(\mathcal{U}^{(1)}\in \mathbb{R}^{R_1 \times D_1 \times D_2 \times R_2})
\]
\[
\mathcal{Z}^{(3)}_{h_2, w_2, r_4, r_1} = \sum_{d_1=1}^{D_1} \sum_{d_2=1}^{D_2} \sum_{s'=1}^1 \sum_{r_2=1}^{R_2}
\tilde{\mathcal{Z}}^{(2)}_{h'_2,w'_2, r_4, r_2 }\mathcal{T}^{(1)}_{d_1, d_2, s', r_2, r_1}
\]
\[
\tilde{\mathcal{Z}}^{(3)} \in \mathbb{R}^{H_2 \times W_2 \times R_1 \times R_4}=
\text{reshape}(\mathcal{Z}^{(3)} \in \mathbb{R}^{H_2 \times W_2 \times R_4 \times R_1})
\]
&
\[\text{Conv-3D}\]
\[D_1 \times D_2 \times 1 \times R_2 \times R_1\]
\[S = (s,s,1)\]
\[P = (p,p,0)\]
&
\[H_2W_2R_4R_1D_1D_2R_2\]\\
\hline
%layer 4
\[
\mathcal{T}^{(4)}\in \mathbb{R}^{1\times 1\times 1\times R_4 \times F_{21}R_5}=
\text{reshape}(\mathcal{U}^{(4)}\in \mathbb{R}^{R_4 \times F_{21} \times R_5})
\]
\[\mathcal{Z}^{(4)}_{h_2, w_2, r_1, f_{21}r_5} = \sum_{p'=1}^1\sum_{q'=1}^1 \sum_{s'=1}^1 \sum_{r_4=1}^{R_4}
\tilde{\mathcal{Z}}^{(3)}_{h_2, w_2, r_1, r_4}\mathcal{T}^{(4)}_{p',q',s', r_4, f_{21}r_5}\]
\[
\tilde{\mathcal{Z}}^{(4)}\in \mathbb{R}^{H_2 \times W_2 \times F_{21} \times R_1R_5} =
\text{reshape}(\mathcal{Z} \in \mathbb{R}^{H_2 \times W_2 \times R_1 \times F_{21}R_5})
\]
&
\[\text{Conv-3D}\]
\[1\times 1 \times 1 \times R_4 \times F_{21}R_5\]
\[S=(1,1,1)\]
\[P=(0,0,0)\]
&
\[H_2W_2R_1F_{21}R_5R_4\]
\\
\hline
%layer 5
\[
\mathcal{T}^{(5)}\in \mathbb{R}^{1\times 1\times 1 \times R_1R_5 \times F_{22}} =
\text{reshape}(\mathcal{U}^{(5)}\in \mathbb{R}^{R_5 \times F_{22}\times R_1})
\]
\[
\mathcal{Z}^{(5)}_{h_2, w_2, f_{21}, f_{22}} = 
\sum_{p'=1}^1 \sum_{q'=1}^1 \sum_{s'=1}^1 \sum_{r_1r_5=1}^{R_1R_5}
\tilde{\mathcal{Z}}^{(4)}_{h_2, w_2, f_{21}, r_1r_5}
\mathcal{T}^{(5)}_{p', q', s', r_1r_5, f_{22}}
\]
\[
\tilde{\mathcal{Z}}^{(5)} \in \mathbb{R}^{H_2 \times W_2 \times F_{21}F_{22}} =
\text{reshape}(\mathcal{Z}^{(5)} \in \mathbb{R}^{H_2 \times W_2 \times F_{21} \times F_{22}})
\]
&
\[\text{Conv-3D}\]
\[1\times 1 \times 1 \times R_1R_5 \times F_{22}\]
\[S=(1,1,1)\]
\[P=(0,0,0)\]
&
\[H_2W_2F_{21}F_{22}R_1R_5\]
\\
\hline
\end{tabular}
\centering
 \caption{High order reshaped tensor ring nets analysis.}
 \label{table: conv_reshape}
 \vspace{-.1in}
 \end{table*}

==> Table_FC_reshape.tex <==
\begin{table*}[t!]
\begin{tabular}{ |p{9.5cm}||p{3.5cm}|p{3cm}|  }
 \hline
 \multicolumn{3}{|c|}{Fully-connected layer in tensor ring nets} \\
 \hline
\[ \text{Formula} \]            			& \[ \text{Method} \] 		& \[ \text{Computation} \]  		 	 \\
 \hline
 % layer 1
 \[
 \mathcal{T}^{(2)}\in \mathbb{R}^{F_{12} \times R_2R_3} = \text{reshape}(\mathcal{U}^{(2)} \in \mathbb{R}^{R_2 \times F_{12} \times R_3})
 \]
\[
\mathcal{Z}^{(1)}_{f_{11}, r_2r_3} = \sum_{f_{12}}\mathcal{X}_{f_{11}, f_{12}} \mathcal{T}^{(2)}_{f_{12}, r_2r_3}
\]
\[
 \tilde{\mathcal{Z}}^{(1)} \in \mathbb{R}^{R_3 \times F_{11}R_2} = \text{reshape}(\mathcal{Z}^{(1)} \in \mathbb{R}^{F_{11} \times R_2R_3})
\]
& \[\text{Fully connected layer}\] 
\[F_{12} \times R_2R_3\] 
&\[ F_{11}F_{12}R_2R_3\]
\\
\hline
\[
\mathcal{T}^{(1)} \in \mathbb{R}^{F_{11}R_2 \times R_1}=
\text{reshape}(\mathcal{U}^{(1)} \in \mathbb{R}^{R_1 \times F_{11} \times R_2})
\]
\[
\mathcal{Z}^{(2)} _{r_3, r_1} = \sum_{f_{11}r_2}^{F_{11}R_2}
\tilde{\mathcal{Z}}^{(1)}_{r_3, f_{11}r_2} \mathcal{T}^{(1)}_{f_{11}r_2, r_1}
\]
\[
\tilde{\mathcal{Z}}^{(2)} \in \mathbb{R}^{R_1 \times R_3} = \text{reshape}(\mathcal{Z}^{(2)} \in \mathbb{R}^{R_3\times R_1})
\]
&
\[\text{Fully connected layer}\]
\[F_{11}R_2 \times R_1\]
&
\[R_3R_1F_{11}R_2\]\\
\hline
\[\mathcal{T}^{(3)} \in \mathbb{R}^{R_3 \times F_{21}R_4} =
\text{reshape}(\mathcal{U}^{(3)} \in \mathbb{R}^{R_3\times F_{21}\times R_4})\]
\[
\mathcal{Z}^{(3)}_{r_1, f_{21}r_4} = \sum_{r_3=1}^{R_3}\tilde{\mathcal{Z}}^{(2)}_{r_1, r_3}\mathcal{T}^{(3)}_{r_3, f_{21}r_4}
\]
\[
\tilde{\mathcal{Z}}^{(3)}\in \mathbb{R}^{F_{21} \times R_4R_1} = \text{reshape}(\mathcal{Z}^{(3)} \in \mathbb{R}^{R_1 \times F_{21}R_4})
\]
&
\[\text{Fully connected layer}\]
\[R_3 \times F_{21}R_4\]
&
\[R_1F_{21}R_4R_3\]\\
\hline
\[
\mathcal{T}^{(4)}\in \mathbb{R}^{R_4R_1 \times F_{22}}=
\text{reshape}(\mathcal{U}^{(4)} \in \mathbb{R}^{R_4 \times F_{22}\times R_1})
\]
\[
\mathcal{Z}^{(4)}_{f_{21}, f_{22}}=\sum_{r_4r_1=1}^{R_4R_1}
\tilde{\mathcal{Z}}^{(3)}_{f_{21}, r_4r_1}
\mathcal{T}^{(4)}_{r_4r_1,f_{22}}
\]
&
\[\text{Fully connected layer}\]
\[R_4R_1 \times F_{22}\]
&
\[F_{21}F_{22}R_4R_1\]
\\
\hline
\end{tabular}
\centering
 \caption{Fully-connected tensor ring layer.}
 \label{table: fc_reshape}
 \vspace{-.1in}
 \end{table*}

==> tikz_figures/DifferentModel.tex <==
\begin{figure*}
\begin{minipage}[b]{0.55\textwidth}	
\begin{subfigure}[b]{0.3\textwidth}
	\begin{tikzpicture} [scale=0.6]   
		\node[draw, shape=circle, scale = .55]  (c) at (0,-4) {$\sigma^{(i)}$};
    		\node[draw, shape=circle, scale = .55] (v1) at (-2.5,-4) {${\bf u}^{(i)}_1$};
    		\node[draw, shape=circle, scale = .55] (v2) at (-1,-2) {${\bf u}^{(i)}_2$};
    		\node[draw, shape=circle, scale = .55] (v3) at (1,-2) {${\bf u}^{(i)}_3$};
    		\node[draw, shape=circle, scale = .55] (v4) at (2.5,-4) {${\bf u}^{(i)}_4$};
    		\node[draw, shape=circle, scale = .55] (v5) at (1,-6) {${\bf u}^{(i)}_5$};
    		\node[draw, shape=circle, scale = .55] (v6) at (-1,-6) {${\bf u}^{(i)}_6$};
    		% rank edge
    		\draw [dashed] (v1) --   node[below] {1}(v2);
    		\draw [dashed] (v2) --   node[below] {1}(v3);
    		\draw [dashed] (v3) --   node[below] {1}(v4);
    		\draw [dashed] (v4) --   node[below] {1}(v5);
    		\draw [dashed] (v5) --   node[below] {1}(v6);
    		\draw [dashed] (v6) --   node[below] {1}(v1);
		% center
		\draw [dashed] (c) --   node[below] {1}(v2);
    		\draw [dashed] (c) --   node[below] {1}(v3);
   		\draw [dashed] (c) --   node[below] {1}(v4);
    		\draw [dashed] (c) --   node[below] {1}(v5);
    		\draw [dashed] (c) --   node[below] {1}(v6);
    		\draw [dashed] (c) --   node[below] {1}(v1);
    		% dangle
    		\draw [thick] (-2.9, -4) --node[above] {$I_1$} (-3.5, -4);
    		\draw [thick] (-1.2, -1.6) --node[left] {$I_2$} (-1.6, -0.8);
    		\draw [thick] (1.2, -1.6) --node[left] {$I_3$} (1.6, -0.8);
    		\draw [thick] (2.9, -4) --node[above] {$I_4$} (3.5, -4);
    		\draw [thick] (1.2, -6.4) --node[right] {$I_5$} (1.6, -7.2);
    		\draw [thick] (-1.2, -6.4) --node[left] {$I_6$} (-1.6, -7.2);
	\end{tikzpicture}
	\caption{CP Decomposition}
	\centering
\end{subfigure} 	
\hspace{.7in}
\begin{subfigure}[b]{0.3\textwidth}
		\begin{tikzpicture}[scale=0.6]    
    		\node[draw, shape=circle, scale = .7] (v1) at (-2.5,-4) {${\bf U}_1$};
    		\node[draw, shape=circle, scale = .7] (v2) at (-1,-2) {$\mathcal{U}_2$};
    		\node[draw, shape=circle, scale = .7] (v3) at (1,-2) {$\mathcal{U}_3$};
    		\node[draw, shape=circle, scale = .7] (v4) at (2.5,-4) {$\mathcal{U}_4$};
    		\node[draw, shape=circle, scale = .7] (v5) at (1,-6) {$\mathcal{U}_5$};
    		\node[draw, shape=circle, scale = .7] (v6) at (-1,-6) {${\bf U}_6$};
    		% rank edge
    		\draw [thick] (v1) --   node[below] {r}(v2);
    		\draw [thick] (v2) --   node[below] {r}(v3);
    		\draw [thick] (v3) --   node[below] {r}(v4);
    		\draw [thick] (v4) --   node[below] {r}(v5);
    		\draw [thick] (v5) --   node[below] {r}(v6);
    		% dangle
    		\draw [thick] (-2.9, -4) --node[below] {$I_1$} (-3.5, -4);
    		\draw [thick] (-1.2, -1.6) --node[left] {$I_2$} (-1.6, -0.8);
    		\draw [thick] (1.2, -1.6) --node[left] {$I_3$} (1.6, -0.8);
    		\draw [thick] (2.9, -4) --node[below] {$I_4$} (3.5, -4);
    		\draw [thick] (1.2, -6.4) --node[left] {$I_5$} (1.6, -7.2);
    		\draw [thick] (-1.2, -6.4) --node[left] {$I_6$} (-1.6, -7.2);
	\end{tikzpicture}
	\caption{TT Decomposition}
	\centering
\end{subfigure} 	

\begin{subfigure}[b]{0.3\textwidth}
	\begin{tikzpicture}[scale=0.6]    
    		\node[draw, shape=circle, scale = .7] (v1) at (-2.5,-4) {$\mathcal{U}_1$};
    		\node[draw, shape=circle, scale = .7] (v2) at (-1,-2) {$\mathcal{U}_2$};
    		\node[draw, shape=circle, scale = .7] (v3) at (1,-2) {$\mathcal{U}_3$};
    		\node[draw, shape=circle, scale = .7] (v4) at (2.5,-4) {$\mathcal{U}_4$};
    		\node[draw, shape=circle, scale = .7] (v5) at (1,-6) {$\mathcal{U}_5$};
    		\node[draw, shape=circle, scale = .7] (v6) at (-1,-6) {$\mathcal{U}_6$};
    		% rank edge
    		\draw [thick] (v1) --   node[below] {$r_1$}(v2);
    		\draw [thick] (v2) --   node[below] {$r_2$}(v3);
    		\draw [thick] (v3) --   node[below] {$r_3$}(v4);
    		\draw [thick] (v4) --   node[below] {$r_4$}(v5);
    		\draw [thick] (v5) --   node[below] {$r_5$}(v6);
    		\draw [thick] (v6) --   node[below] {$r_6$}(v1);
    		% dangle
    		\draw [thick] (-2.9, -4) --node[below] {$I_1$} (-3.5, -4);
    		\draw [thick] (-1.2, -1.6) --node[left] {$I_2$} (-1.6, -0.8);
    		\draw [thick] (1.2, -1.6) --node[left] {$I_3$} (1.6, -0.8);
    		\draw [thick] (2.9, -4) --node[below] {$I_4$} (3.5, -4);
    		\draw [thick] (1.2, -6.4) --node[left] {$I_5$} (1.6, -7.2);
    		\draw [thick] (-1.2, -6.4) --node[left] {$I_6$} (-1.6, -7.2);
	\end{tikzpicture}
	\caption{TR Decomposition}
	\centering
\end{subfigure} 
\hspace{.7in}
\begin{subfigure}[b]{0.4\textwidth}
	\begin{tikzpicture}[scale=0.6]    
    		\node[draw, shape=circle, scale = .7] (v1) at (-2.5,-4) {${\bf U}_1$};
    		\node[draw, shape=circle, scale = .7] (v2) at (-1,-2) {${\bf U}_2$};
    		\node[draw, shape=circle, scale = .7] (v3) at (1,-2) {${\bf U}_3$};
    		\node[draw, shape=circle, scale = .7] (v4) at (2.5,-4) {${\bf U}_4$};
    		\node[draw, shape=circle, scale = .7] (v5) at (1,-6) {${\bf U}_5$};
    		\node[draw, shape=circle, scale = .7] (v6) at (-1,-6) {${\bf U}_6$};
    		\node[draw, shape=circle, scale = .7] (c)   at(0, -4) {$\mathcal{C}$};
    		% center
    		\draw [thick] (c) --   node[below] {c}(v2);
    		\draw [thick] (c) --   node[below] {c}(v3);
   		\draw [thick] (c) --   node[below] {c}(v4);
    		\draw [thick] (c) --   node[below] {c}(v5);
    		\draw [thick] (c) --   node[below] {c}(v6);
    		\draw [thick] (c) --   node[below] {c}(v1);
    		% dangle
    		\draw [thick] (-2.9, -4) --node[below] {$I_1$} (-3.5, -4);
    		\draw [thick] (-1.2, -1.6) --node[left] {$I_2$} (-1.6, -0.8);
    		\draw [thick] (1.2, -1.6) --node[left] {$I_3$} (1.6, -0.8);
    		\draw [thick] (2.9, -4) --node[below] {$I_4$} (3.5, -4);
    		\draw [thick] (1.2, -6.4) --node[left] {$I_5$} (1.6, -7.2);
    		\draw [thick] (-1.2, -6.4) --node[left] {$I_6$} (-1.6, -7.2);
	\end{tikzpicture}
	\caption{Turcker Decomposition}
	\centering
\end{subfigure}
\end{minipage} 
\hspace{.2in}
\begin{subfigure}[b]{0.35\textwidth}
	\begin{tikzpicture}[scale=.8]    
    		\node[draw, shape=circle, scale = .7] (v1) at (-2.5,-4) {$\mathcal{U}_1$};
    		\node[draw, shape=circle, scale = .7] (v2) at (-1,-2) {$\mathcal{U}_2$};
    		\node[draw, shape=circle, scale = .7] (v3) at (1,-2) {$\mathcal{U}_3$};
    		\node[draw, shape=circle, scale = .7] (v4) at (2.5,-4) {$\mathcal{U}_4$};
    		\node[draw, shape=circle, scale = .7] (v5) at (1,-6) {$\mathcal{U}_5$};
    		\node[draw, shape=circle, scale = .7] (v6) at (-1,-6) {$\mathcal{U}_6$};
    		\node[draw, shape=circle, scale = .7] (c)   at(0, -4) {$\mathcal{C}$};
    		% rank edge
    		\draw [thick] (v1) --   node[below] {r}(v2);
    		\draw [thick] (v2) --   node[below] {r}(v3);
    		\draw [thick] (v3) --   node[below] {r}(v4);
    		\draw [thick] (v4) --   node[below] {r}(v5);
    		\draw [thick] (v5) --   node[below] {r}(v6);
    		\draw [thick] (v6) --   node[below] {r}(v1);
    		% center
    		\draw [thick] (c) --   node[below] {c}(v2);
    		\draw [thick] (c) --   node[below] {c}(v3);
   		\draw [thick] (c) --   node[below] {c}(v4);
    		\draw [thick] (c) --   node[below] {c}(v5);
    		\draw [thick] (c) --   node[below] {c}(v6);
    		\draw [thick] (c) --   node[below] {c}(v1);
    		% dangle
    		\draw [thick] (-2.9, -4) --node[below] {$I_1$} (-3.5, -4);
    		\draw [thick] (-1.2, -1.6) --node[left] {$I_2$} (-1.6, -0.8);
    		\draw [thick] (1.2, -1.6) --node[left] {$I_3$} (1.6, -0.8);
    		\draw [thick] (2.9, -4) --node[below] {$I_4$} (3.5, -4);
    		\draw [thick] (1.2, -6.4) --node[left] {$I_5$} (1.6, -7.2);
    		\draw [thick] (-1.2, -6.4) --node[left] {$I_6$} (-1.6, -7.2);
	\end{tikzpicture}
	\vspace{.8in}
	\caption{TuR Decomposition}
	\centering
\end{subfigure} 	
\caption{Tensor network representation for a $6$-order tensor via Canonical Polyadic (CP) decomposition, Tensor Train (TT) decomposition, Tensor Ring (TR) decomposition, Tucker decomposition, and Tucker Ring (TuR) decomposition.{\bf Each node represents a tensor and the amount of edges connected a node represents the tensor order. The value on the edge is the dimension of the tensor mode, where a mode with dimension $1$ can either be added or removed.} Solid edges have dimension larger than $1$ while dashed edges have dimension $1$.}
\label{TN_figure}
\vspace{-.1in}
\end{figure*}
\begin{table*}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{ |c||c|c|c|  }
 %\hline
 %\multicolumn{4}{|c|}{Cifar10} \\
 \hline
 Method            	&Entry$\left( T(i_1,\cdots, i_d) \right)$ 	& Storage 			& DoF  \\
  \hline
CP 					& $\sum_i \sigma^{(i)} {\bf u}_1^{(i)}(i_1) \cdots {\bf u}_d^{(i)}(i_d)$				& $dIr + r$  		  	&  -\\	
  \hline
TT					& $\sum_{r_1, \cdots, r_{d-1}}{\bf U}_1(i_1, r_1)\mathcal{U}_2(r_1, i_2, r_2) \cdots \mathcal{U}_{d-1}(r_{d-2}, i_{d-1}, r_{d-1}) {\bf U}_d(r_{d-1},i_d)$ 				& $(d-2)Ir^2 + 2Ir$ 		& $(d-2)(Ir^2-r^2) + (2Ir -r^2)$  \\
 \hline
 TR  					& $\sum_{r_0,r_1, \cdots, r_{d-1}}\mathcal{U}_1(r_0, i_1, r_1) \cdots \mathcal{U}_{d}(r_{d-1}, i_{d}, r_{0})$ 				& $dIr^2$   			&  - \\
 \hline
 Tucker				& $\sum_{r_1,\cdots, r_d} {\bf U}_1(i_1, r_1)\cdots {\bf U}_d(i_d, r_d) \mathcal{C}(r_1,\cdots, r_d)$				& $dIr + r^d$ 			&  $d(Ir-r^2) + r^d$  \\
 \hline
 TuR					& $\sum_{r_0,\cdots, r_{d-1}, c_1,\cdots, c_d} \mathcal{U}_1(r_0, i_1, r_1, c_1) \cdots \mathcal{U}_d(r_{d-1}, i_d, r_0, c_d) \mathcal{C}(c_1,\cdots, c_d)$				& $cdIr^2 + c^d$ 		&  -  \\
\hline
\end{tabular}
\end{adjustbox}
\centering
\caption{ Comparison of CP, TT, TR, Tucker, and TuR decomposition in entry representation, storage, and Degree of Freedom(DoF). }
\vspace{-.1in}
\label{TN_table}
\end{table*}









==> tikz_figures/FullyConnected.tex <==
\begin{figure}[t]
\begin{tikzpicture}
    \node[draw, shape=circle] (v0) at (0,0) {$\mathscr{X}^{(\ell)}$};
    \node[draw, shape=circle] (v1) at (-2.5,-2) {$\mathscr{U}_1^{(\ell)}$};
    \node[draw, shape=circle] (v2) at (-1,-2) {$\mathscr{U}_2^{(\ell)}$};
    \node[draw, shape=circle] (v3) at (1,-2) {$\mathscr{U}_3^{(\ell)}$};
    \node[draw, shape=circle] (v4) at (2.5,-2) {$\mathscr{U}_4^{(\ell)}$};
    \node[draw, shape=circle] (v11) at (-2.5,-4) {$\mathscr{U}_1^{(\ell)}$};
    \node[draw, shape=circle] (v12) at (-1,-4) {$\mathscr{U}_2^{(\ell)}$};
    \node[draw, shape=circle] (v13) at (1,-4) {$\mathscr{U}_3^{(\ell)}$};
    \node[draw, shape=circle] (v14) at (2.5,-4) {$\mathscr{U}_4^{(\ell)}$};
    % output edge
    \draw[thick, label=below:{v14}] (-2.5,-4.55) -- node[left] {$I_1^{(\ell+1)}$} (-2.5,-5.5); 
    \draw[thick, label=below:{v13}] (-1,-4.55) --    node[left] {$I_2^{(\ell+1)}$}  (-1,-5.5);
    \draw[thick, label=below:{v12}] (1,-4.55) --     node[left] {$I_3^{(\ell+1)}$}(1,-5.5);
    \draw[thick, label=below:{v11}] (2.5,-4.55) --  node[left] {$I_4^{(\ell+1)}$}(2.5,-5.5);
    \draw[thick, label=above:{v0}] (0,.5) --  node[left] {$n$}(0,1.5);
    % input edge
    \draw [thick] (v0) -- node[left] {$I_1^{(\ell)}$} (v1);
    \draw [thick] (v0) -- node[left] {$I_2^{(\ell)}$}(v2);
    \draw [thick] (v0) -- node[left] {$I_3^{(\ell)}$}(v3); 
    \draw [thick] (v0) -- node[left] {$I_4^{(\ell)}$}(v4);
    % rank edge
    \draw [thick] (v1) --   node[below] {r}(v2);
    \draw [thick] (v2) --   node[below] {r}(v3);
    \draw [thick] (v3) --   node[below] {r}(v4);
    \draw [thick] (v4) --   node[left]      {r}(v14);
    \draw [thick] (v11) -- node[above] {r}(v12);
    \draw [thick] (v12) -- node[above] {r}(v13);
    \draw [thick] (v13) -- node[above] {r}(v14);
    \draw [thick] (v11) --  node[right] {r} (v1) ;   
    {\color{green}
    % mark W
    \draw[dashed, label=below:{v11}] (-3.5, -1.4) -- (3.2, -1.4);
    \draw[dashed, label=below:{v11}] (-3.5, -1.4) -- (-3.5, -4.6);
    \draw[dashed, label=below:{v11}] (-3.5, -4.6) -- (3.2, -4.6);
    \draw[dashed, label=below:{v11}] (3.2, -4.6) --  node[right] {$\mathscr{W}^{(\ell)}$}(3.2, -1.4);
    }
    % mark X_l
    {\color{blue}
    \draw[dashed, label=below:{v11}] (-3.5, 1.6) -- (3.2, 1.6);
    \draw[dashed, label=below:{v11}] (-3.5, -.6) -- (-3.5, 1.6);
    \draw[dashed, label=below:{v11}] (-3.5, -.6) -- (3.2, -.6);
    \draw[dashed, label=below:{v11}] (3.2, -.6) --  node[right] {$\mathscr{X}^{(\ell)}$}(3.2,1.6);
    }
    % mark X_l+1
     {\color{red}
    \draw[dashed, label=below:{v11}] (-3.7, 1.7) -- (4.1, 1.7);
    \draw[dashed, label=below:{v11}] (-3.7, -5.3) -- (-3.7, 1.7);
    \draw[dashed, label=below:{v11}] (-3.7, -5.3) -- (4.1, -5.3);
    \draw[dashed, label=below:{v11}] (4.1, -5.3) --  node[right] {$\mathscr{X}^{(\ell+1)}$}(4.1, 1.7);
    }
    \end{tikzpicture}
 \centering
 \caption{Tensor Network Representation: FC-TRN($d=4$). 
    %$\mathscr{W}^{(\ell)} \in \mathbb{R}^{I_1^{(\ell)} \times I_2^{(\ell)} \times I_3^{(\ell)} \times I_4^{(\ell)} \times I_1^{(\ell + 1)} \times I_2^{(\ell + 1)} \times I_3^{(\ell + 1)} \times I_4^{(\ell + 1)} }$, 
    %$\mathscr{X}^{(\ell)} \in \mathbb{R}^{_1^{(\ell)} \times I_2^{(\ell)} \times I_3^{(\ell)} \times I_4^{(\ell)}}$ ,
    %$\mathscr{X}^{(\ell+1)} \in \mathbb{R}^{_1^{(\ell+1)} \times I_2^{(\ell+1)} \times I_3^{(\ell+1)} \times I_4^{(\ell+1)}}$
    }
 \label{FC}
 \vspace{-.2in}
\end{figure}

==> tikz_figures/TuckerRing_Figure.tex <==
\begin{figure}[t]
	%\begin{subfigure}[b]{0.3\textwidth}
	\begin{tikzpicture}    
    		\node[draw, shape=circle] (v1) at (-2.5,-4) {$\mathcal{U}_1$};
    		\node[draw, shape=circle] (v2) at (-1,-2) {$\mathcal{U}_2$};
    		\node[draw, shape=circle] (v3) at (1,-2) {$\mathcal{U}_3$};
    		\node[draw, shape=circle] (v4) at (2.5,-4) {$\mathcal{U}_4$};
    		\node[draw, shape=circle] (v5) at (1,-6) {$\mathcal{U}_5$};
    		\node[draw, shape=circle] (v6) at (-1,-6) {$\mathcal{U}_6$};
    		\node[draw, shape=circle] (c)   at(0, -4) {$\mathcal{C}$};
    		% rank edge
    		\draw [thick] (v1) --   node[below] {r}(v2);
    		\draw [thick] (v2) --   node[below] {r}(v3);
    		\draw [thick] (v3) --   node[below] {r}(v4);
    		\draw [thick] (v4) --   node[below] {r}(v5);
    		\draw [thick] (v5) --   node[below] {r}(v6);
    		\draw [thick] (v6) --   node[below] {r}(v1);
    		% center
    		\draw [thick] (c) --   node[below] {c}(v2);
    		\draw [thick] (c) --   node[below] {c}(v3);
   		\draw [thick] (c) --   node[below] {c}(v4);
    		\draw [thick] (c) --   node[below] {c}(v5);
    		\draw [thick] (c) --   node[below] {c}(v6);
    		\draw [thick] (c) --   node[below] {c}(v1);
    		% dangle
    		\draw [thick] (-2.9, -4) --node[below] {$I_1$} (-3.5, -4);
    		\draw [thick] (-1.2, -1.6) --node[left] {$I_2$} (-1.6, -0.8);
    		\draw [thick] (1.2, -1.6) --node[left] {$I_3$} (1.6, -0.8);
    		\draw [thick] (2.9, -4) --node[below] {$I_4$} (3.5, -4);
    		\draw [thick] (1.2, -6.4) --node[left] {$I_5$} (1.6, -7.2);
    		\draw [thick] (-1.2, -6.4) --node[left] {$I_6$} (-1.6, -7.2);
	\end{tikzpicture}
	%\end{subfigure}
\caption{Tucker Ring Decomposition.}
\label{TuR}
 \vspace{-.2in}
\end{figure}
